Multi-output multilevel best linear unbiased estimators via semidefinite programming

Multifidelity forward uncertainty quantification (UQ) problems often involve multiple quantities of interest and heterogeneous models (e.g., different grids, equations, dimensions, physics, surrogate and reduced-order models). While computational efficiency is key in this context, multi-output strategies in multilevel/multifidelity methods are either sub-optimal or non-existent. In this paper we extend multilevel best linear unbiased estimators (MLBLUE) to multi-output forward UQ problems and we present new semidefinite programming formulations for their optimal setup. Not only do these formulations yield the optimal number of samples required, but also the optimal selection of low-fidelity models to use. While existing MLBLUE approaches are single-output only and require a non-trivial nonlinear optimization procedure, the new multi-output formulations can be solved reliably and efficiently. We demonstrate the efficacy of the new methods and formulations in practical UQ problems with model heterogeneity.

==> Makefile <==
default:
	pdflatex -shell-escape arxiv
	bibtex arxiv
	pdflatex -shell-escape arxiv
	pdflatex -shell-escape arxiv

clean:
	rm *~ *.aux *.out *.toc *.blg *.bbl *.log *.tdo *.pag

diff:
	cp arxiv.tex arxiv_new.tex
	git checkout 9e644d145395c8fb7aad66db5399c18c315bb341 -- arxiv.tex
	cp arxiv.tex arxiv_old.tex
	git reset HEAD
	cp arxiv_new.tex arxiv.tex
	latexdiff --packages=hyperref arxiv_old.tex arxiv_new.tex > diff.tex
	sed -i '/\\fi/a \\\renewcommand{\\limits}{}' diff.tex
	sed -i '/\\fi/a \\\DeclareMathOperator{\\D}{\\mathcal{D}}' diff.tex
	pdflatex diff.tex
	bibtex diff.aux
	pdflatex diff.tex
	pdflatex diff.tex


